Reflection-Window Decoding: Text Generation with Selective Refinement

The autoregressive decoding for text generation in large language models (LLMs), while widely used, is inherently suboptimal due to the lack of a built-in mechanism to perform refinement and/or correction of the generated content. In this paper, we consider optimality in terms of the joint probability over the generated response, when jointly considering all tokens at the same time. We theoretically characterize the potential deviation of the autoregressively generated response from its globally optimal counterpart that is of the same length. Our analysis suggests that we need to be cautious when noticeable uncertainty arises during text generation, which may signal the sub-optimality of the generation history. To address the pitfall of autoregressive decoding for text generation, we propose an approach that incorporates a sliding reflection window and a pausing criterion, such that refinement and generation can be carried out interchangeably as the decoding proceeds. Our selective refinement framework strikes a balance between efficiency and optimality, and our extensive experimental results demonstrate the effectiveness of our approach.

==> file/main/method.tex <==
\section{Related Works}

In this section, we will discuss LLMs Self-Correction, Reinforcement Learning, and Combinatorial Optimization. 

\textbf{LLMs Self-correction.} \ Self-correction can be categorized into 2 parts, from internal feedback to external feedback. In this paper, we intend to train a model as external feedback to tell the LLM where the previous tokens are most likely to be wrong. 

\textbf{Combinatorial Optimization and Reinforcement Learning.} \ In our paper we formulate the problematic interval finding as a combinatorial optimization problem. If there are multiple problematic intervals with varying lengths in the past $n$ tokens, then the complexity of finding all those intervals will be NP-hard. This is similar to the delaunay triangulation problem. 

\section{Selective Refinement via Reinforcement Learning}

We train our selective refinement model with reinforcement learning, and here we explain the definition of our state, action, and policy.

RL Definition and  

==> file/parking/MTBench_winrate.tex <==
% \begin{table*}[t]
%     \centering
%     \newcolumntype{g}{>{\columncolor{Gray}}c}
%     \caption{Win Rate Against Greedy Decoding on MT-Bench}
%     \label{tab:table2}
%     \begin{tabular}{lccccc}
%         \toprule
%         \textbf{Method}   & \textbf{Win} & \textbf{Lose} & \textbf{Tie} & \textbf{Win rate} \\
%         \midrule
%         % Greedy Sampling &  &   &   &    \\
%         Beam Search       & 25           & 29            & 26           & 46.30\%           \\
%         Reflection Window & 26           & 13            & 41           & \textbf{66.67\%}  \\
%         \bottomrule
%     \end{tabular}
%     % \setlength{\abovecaptionskip}{-0.1cm}
% \end{table*}

\begingroup
\renewcommand{\arraystretch}{1}
\begin{table}[t]
    \caption{Win Rate Against Greedy Decoding on MT-Bench}
    \label{tab:table2}
    \centering
    \footnotesize
    \begin{tabular}{L{0.18}C{0.06}C{0.07}C{0.06}C{0.09}}
        \toprule
        \textbf{Method} & \textbf{Win} & \textbf{Lose} & \textbf{Tie} & \textbf{Rate} \\
        \midrule
        Beam Search & 25 & 29 & 26 & 46.30\% \\
        Reflection-Window & 26 & 13 & 41 & \textbf{66.67\%} \\
        \bottomrule
    \end{tabular}
\end{table}
\endgroup

==> file/parking/formulation.comment.tex <==
\section{Formulation}\label{main:formulation}

Just an example of reference in cognitive linguistics \citep{fedorenko2024language}.

\subsection{High-Level Picture}
The goal of this project is to incorporate following characteristics during text generating:
\begin{enumerate}
    \item going beyond autoregressive way of text generation, explicitly introduce the selection mechanism among generated text, where the conditions under which the (final) objective/target/expectation/goal is achieve are specified by the prompt
    \item enable the ability to reflect on generated text as the generation goes on, always with the target in mind (analogous to human writing, where we constantly reflect on what was written, and whether we are \emph{approaching} the goal as we proceed)
    \item a mechanism that is not too heavy to be practically operationalizable
\end{enumerate}

There are two different modules: (1) the criterion that specifies whether we are \emph{approaching} our final goal, and (2) the mechanism that allows LLM to always reflect on what was generated and to decide whether revision is necessary to ensure we are getting closer and closer to our goal (according to the aforementioned criterion).


\subsection{Reflection Window}
Considering the fact that the text typically flows in a single dimension, i.e., from the start to the end, there is an intrinsic linear structure (of words, phrases, and sentences) in text generation.
This linear structure differentiates text from other forms of objects that occupy multiple dimensional spaces, e.g., images or videos, which can be perceived from multiple angles.
Therefore, taking advantage of this linear structure, we propose a sliding window mechanism to perform text generation and reflection at the same time as the output unfolds.

There are position indices, let us call them fast index and slow index.\footnote{
    The naming of them is motivated by \citet{kahneman2011thinking}.
}
Let us denote the text between \texttt{<START>} and the slow index as $A$, the content between slow and fast indices as $B$, and the immediate token after the fast indices as $C$.
Let us denote the goal (currently, use the prompt/instruction itself as the surrogate) as $G_{\mathrm{raw}}$, and its paraphrased mission-complete version as $G_{\mathrm{success}}$.
For instance, if $G_{\mathrm{raw}}$ is ``tell a joke,'' then $G_{\mathrm{success}}$ can be ``the generated text tells a joke.''
The reason of having these two versions is to have a way to evaluate the generated content and see if we are approaching the goal.

When slow index does not forward, and only the fast index is moving forward (generating mode)
\begin{equation}
    \begin{split}
        B & \leftarrow (B, C) \\
        C & \leftarrow C'
    \end{split}
\end{equation}

When fast index is paused, and only the slow index is trying to locate the problematic part in generated text (reflecting mode)
\begin{equation}
    \begin{split}
        A & \leftarrow (A, B[0]) \\
        B & \leftarrow B[1:]
    \end{split}
\end{equation}

Notice that the reflection window mechanism does not require the completion of the entire LLM output before the reflection can kick in.
This is favorable (compared to post-processing the generated output) since (let us consider the human writing analogy) for several reasons.
To begin with, one do not have to wait until the entire essay to be finished before improving the content.
Furthermore, if there are multiple potential issues (in the sense of deviating from the goal) in the writing, the revision can be unnecessarily demanding (in the sense that we need to operate on a more coarse granularity, e.g., regenerate at the sentence level rather than phrase level) and we will have to perform multiple iterations of editing.


\subsection{Stopping Criterion}
Let us denote a token from the vocabulary $\Vcal$ as $w_v \in \Vcal$, whose index in the vocabulary is $v \in \lvert \Vcal \rvert$.

\begin{definition}[Stepwise Optimal length-$T$ Response]
    We say a sequence $w_{\widehat{\vbf}_T[1]} w_{\widehat{\vbf}_T[2]} \ldots w_{\widehat{\vbf}_T[T]}$ is stepwise optimal following the prompt $X_{\leq 0}$, if the sequence consists of tokens that correspond to the highest token-by-token conditional probabilities, denoted by $g(\cdot)$:
    \begin{equation}
        \begin{split}
            \widehat{\vbf}_T[1]          & \coloneqq \argmax_{v_1 \in \lvert \Vcal \rvert} g(X_1 = w_{v_1} \mid X_{\leq 0}),                                                                                                   \\
            \widehat{\vbf}_T[2]          & \coloneqq \argmax_{v_2 \in \lvert \Vcal \rvert} g(X_2 = w_{v_2} \mid X_1 = w_{\widehat{\vbf}_T[1]}, X_{\leq 0}),                                                                    \\
                                         & \ldots                                                                                                                                                                              \\
            \widehat{\vbf}_T[T]          & \coloneqq \argmax_{v_T \in \lvert \Vcal \rvert} g(X_T = w_{v_T} \mid X_{1:T - 1} = w_{\widehat{\vbf}_T[1]} w_{\widehat{\vbf}_T[2]} \ldots w_{\widehat{\vbf}_T[T - 1]}, X_{\leq 0}), \\
            \text{and } \widehat{\vbf}_T & = (\widehat{\vbf}_T[1], \widehat{\vbf}_T[2], \ldots, \widehat{\vbf}_T[T]).
        \end{split}
    \end{equation}
\end{definition}

\begin{definition}[Global Optimal Length-$T$ Response]\label{def:optimal_sequence}
    % \looseness=-1
    We say a sequence $w_{\vbf_T^*[1]} w_{\vbf_T^*[2]} \ldots w_{\vbf_T^*[T]}$ is global optimal among all possible length-$T$ responses following the prompt $X_{\leq 0}$, if it has the highest ground-truth conditional probability, denoted by $f(X_{1:T} \mid X_{\leq 0})$:
    \begin{equation}
        \vbf_T^* = (\vbf_T^*[1], \vbf_T^*[2], \ldots, \vbf_T^*[T]) \coloneqq
        \argmax_{v_i \in \lvert \Vcal \rvert, i=1,2,\ldots,T} f(X_{1:T} = w_{v_1} w_{v_2} \ldots w_{v_T} \mid X_{\leq 0}).
    \end{equation}
\end{definition}

In general, the longer the sequence, the lower the overall probability tends to be.
The fair comparison of optimality is length specific, and the optimal response of a shorter length is not necessarily identical to the prefix of the optimal response that is longer in length.
For instance, if we were to use 10 words to distinguish between joint and conditional densities, one might say ``\emph{joint density combines all variables; conditional adjusts for known outcomes}.''
However, if we can use 15 words, one might say ``\emph{joint density reflects combined probabilities of all variables; conditional density adjusts probabilities given known outcomes}.''
Therefore, we explicitly keep the length $T$ in the notation of vocabulary indices of tokens that constitute the length-$T$ responses.

\begin{assumption}[Well-Trained LLM]\label{aspt:well_trained_LLM}
    We say an autoregressive LLM is well-trained, if the following relation holds for any response of a length $T > 1$:
    \begin{equation}
        f(X_{1:T} \mid X_{\leq 0}) = g(X_1 \mid X_{\leq 0}) ~ \Pi_{t = 1}^{T - 1} g(X_{t + 1} \mid X_{1:t}, X_{\leq 0}).
    \end{equation}
    % where $g(\cdot)$ denotes the conditional probability of autoregressive way of token-by-token generation.
\end{assumption}
Assumption~\ref{aspt:well_trained_LLM} specifies that after given the prompt or generated text history $X_{\leq 0}$, a well-trained LLM can recover the ground-truth probability of $X_{1:T}$ as a whole follows $X_{\leq 0}$, by multiplying token-by-token generating probabilities in an autoregressive way.\footnote{
    Here, we implicitly assume that the context length of the LLM is sufficiently large.
}
We would like to note that Assumption~\ref{aspt:well_trained_LLM} only states that a well-trained LLM can perfectly capture the autoregressive way of probability partitioning of text sequences, and this itself does not guarantee the equivalence of stepwise optimal response and the same-length global optimal response for $T > 1$.
% \footnote{
%     When $T = 1$, this indicates that the LLM outputs \texttt{<eos>} immediately after the prompt, and we omit this case in the discussion.
% }

\begin{assumption}[Irreversible Advantage Once Manifested]\label{aspt:no_return_after_detour}
    When a stepwise optimal length-$T$ response from a well-trained (Assumption~\ref{aspt:well_trained_LLM}) autoregressive LLM $w_{\widehat{\vbf}_T[1]} w_{\widehat{\vbf}_T[2]} \ldots w_{\widehat{\vbf}_T[T]}$ is not the global optimal length-$T$ response $w_{\vbf_T^*[1]} w_{\vbf_T^*[2]} \ldots w_{\vbf_T^*[T]}$, then if the deviation manifest itself at the length-$L$ ($1 \leq L \leq T$) prefix-sequences, the advantage of the global optimal length-$T$ response will not be reversed afterwards:
    \begin{equation*}
        \small
        \begin{split}
             & \text{if }\exists L \in [1, T], f(X_{1:L} = w_{\widehat{\vbf}_T[1]} w_{\widehat{\vbf}_T[2]} \ldots w_{\widehat{\vbf}_T[L]} \mid X_{\leq 0}) < f(X_{1:L} = w_{\vbf_T^*[1]} w_{\vbf_T^*[2]} \ldots w_{\vbf_T^*[L]} \mid X_{\leq 0}), \\
             & \text{then }\forall M \in [L, T], f(X_{1:M} = w_{\widehat{\vbf}_T[1]} \ldots w_{\widehat{\vbf}_T[M]} \mid X_{\leq 0}) < f(X_{1:M} = w_{\vbf_T^*[1]} \ldots w_{\vbf_T^*[M]} \mid X_{\leq 0}).
        \end{split}
    \end{equation*}
\end{assumption}
Assumption~\ref{aspt:no_return_after_detour} specifies that if the advantage (in terms of a higher ground-truth conditional probability) of the global optimal length-$T$ sequence can be observed at the length-$L$ prefix-sequence, such advantage will not be reversed when considering longer prefix-sequences.

\begin{theorem}[Indication of Deviation from the Global Optimal Length-$T$ Response]
    % Suppose that the context length $N$ of LLM is sufficiently large.
    Given the prompt $X_{\leq 0}$, when the well-trained LLM (Assumption~\ref{aspt:well_trained_LLM}) generates a stepwise optimal length-$T$ response which is not the global optimal response with a same length, let $1 < L \leq T$ denote the minimum length of prefix-sequence needed in order for such deviation to manifest itself (Assumption 1.3).
    Then, the conditional probability when generating the token $w_{v_L} \in \Vcal$ is bounded away from $1$ with a positive number $\epsilon_L > 0$, i.e.,
    % In other words, the LLM will be relatively uncertain about
    \begin{equation}
        \begin{split}
            %  & \text{if } L = 1, \text{ then } 1 - \epsilon_1 > \max_{w \in \Vcal} g(X_1 = w \mid X_{\leq 0}),                                                                                                 \\
            %  & \text{if } L > 1,
            \text{ then } 1 - \epsilon_L > \max_{w \in \Vcal} g(X_L = w \mid X_{1:L-1} = w_{\widehat{\vbf}_T[1]} w_{\widehat{\vbf}_T[2]} \ldots w_{\widehat{\vbf}_T[L - 1]}, X_{\leq 0}).
        \end{split}
    \end{equation}
\end{theorem}

\begin{comment}
Since the context length of the LLM is $N$, and the text generation takes a token-by-token format, one can write the conditional probability of generating the next token in terms of a transition probability of a 1-st order Markov process, where the transition is over the enhanced state space of all possible combinations of length-$N$ sequences:
\begin{equation}\label{equ:markov_transition}
    P(\overline{X_{t - N + 2} \ldots X_t} \, X_{t + 1} \mid X_{t - N + 1} \, \overline{X_{t - N + 2} \ldots X_t}) \coloneqq g(X_{t + 1} \mid X_{t - N + 1:t}).
\end{equation}
In the right-hand side of Equation~\ref{equ:markov_transition}, we use the overline notation $\overline{~\cdot~}$ to denote identical sub-sequences before and after state transition.
% The new state $\overline{X_{t - N + 2} \ldots X_t} \, X_{t + 1}$ is the length-$(N - 1)$ suffix of the previous state, i.e., $\overline{X_{t - N + 2} \ldots X_t}$, appended with the newly generated token $X_{t + 1}$.
Here, we are not imposing the assumption that the LLM with a context length of $N$ is a $(N + 1)$-gram model.
Instead, we use the transition matrix of the 1-st order Markov process over the enhanced state space (of length-$N$ sequences) to simplify the notation when characterizing the probability of generating a specific sequence.
Specifically, with a slight abuse of notation, let $\Abf([v_{t - N + 1 : t}]; [v_{t - N + 2 : t + 1}])$ denote entries in the transition matrix, which is indexed by two lists of vocabulary indices that form the from-sequence and to-sequence, respectively.
Let $\pi^{(t)}([v_{t - N + 1 : t}])$ denote the probability of reaching the state $w_{v_{t - N + 1}} w_{v_{t - N + 2}} \ldots w_t$ at the step $t$.

We can use $\pi^{(0)}$ to represent the initial condition specified by the prompt $X_{\leq 0}$ (after processed by the LLM).
Then, the probability of generating the next token $w_{v_{t + 1}}$ is the product of the distribution of states and the transition matrix:
\begin{equation}
    \pi^{(t + 1)}(v_{t - N + 2:t + 1})
    = \sum_{v_{t - N + 1 : t} \in \Vcal^N} \pi^{(t)}(v_{t - N + 1 : t}) \Abf(v_{t - N + 1 : t}; v_{t - N + 2 : t + 1}).
\end{equation}

If the current state is a length-$N$ sequence $X_{t - N + 1} \, \overline{X_{t - N + 2} \ldots X_t}$, then only when the next state starts with the length-$(N-1)$ suffix of the current state can the corresponding entries in the transition matrix to be nonzero.
We can denote with $\hat{v}_{t + 1}$ the index of the newly sampled token, given the previously sampled sequence $w_{\hat{v}_{t - N + 1}} w_{\hat{v}_{t - N + 2}} \ldots w_{\hat{v}_{t}}$:
\begin{equation}
    \hat{v}_{t + 1} = \argmax_{v_{t + 1}} \pi^{(t + 1)}(v_{t - N + 2:t} = \hat{v}_{t - N + 2:t}, v_{t + 1}).
\end{equation}

Since $L$ is the minimum length of prefix-sequence needed in order for the advantage of the global optimal length-$T$ response to manifest, we have:
\begin{equation}
    \begin{split}
        \forall t < L, f(X_{1:t} = w_{\hat{v}_1} w_{\hat{v}_2} \ldots w_{\hat{v}_t} \mid X_{\leq 0}) & > f(X_{1:t} = w_{\vbf^*[1]} w_{\vbf^*[2]} \ldots w_{\vbf^*[t]} \mid X_{\leq 0}), \\
        \text{and } f(X_{1:L} = w_{\hat{v}_1} w_{\hat{v}_2} \ldots w_{\hat{v}_L} \mid X_{\leq 0})    & < f(X_{1:L} = w_{\vbf^*[1]} w_{\vbf^*[2]} \ldots w_{\vbf^*[L]} \mid X_{\leq 0}).
    \end{split}
\end{equation}
In other words,
\begin{equation}
    \big( \pi^{(0)} \Abf \big)(\hat{v}_1) > \big( \pi^{(0)} \Abf \big)(\vbf^*_T[1]),
\end{equation}
\begin{equation}
    \big( \pi^{(1)} \Abf \big)(\hat{v}_1, \hat{v}_2) > \big( \pi^{(1)} \Abf \big)(\vbf^*_T[1], \vbf^*_T[2]),
\end{equation}
\begin{equation*}
    \ldots
\end{equation*}
\begin{equation}
    \big( \pi^{(L - 1)} \Abf \big)(\hat{v}_1, \hat{v}_2, \ldots, \hat{v}_{L - 1}) > \big( \pi^{(L - 1)} \Abf \big)(\vbf^*_T[1], \vbf^*_T[2], \ldots, \vbf^*_T[L - 1]),
\end{equation}
\begin{equation}
    \big( \pi^{(L)} \Abf \big)(\hat{v}_1, \hat{v}_2, \ldots, \hat{v}_L) < \big( \pi^{(L)} \Abf \big)(\vbf^*_T[1], \vbf^*_T[2], \ldots, \vbf^*_T[L]).
\end{equation}

We have
\begin{equation}
    \begin{split}
        \forall v \in \Vcal, & \Abf(\overline{\hat{v}_1, \hat{v}_2, \ldots, \hat{v}_{L - 1}} ; \overline{\hat{v}_1, \hat{v}_2, \ldots, \hat{v}_{L - 1}}, v)
        < \frac{\big( \pi^{(L - 1)} \Abf \big)(\vbf^*_T[1], \vbf^*_T[2], \ldots, \vbf^*_T[L - 1])}{\big( \pi^{(L - 1)} \Abf \big)(\hat{v}_1, \hat{v}_2, \ldots, \hat{v}_{L - 1})} \\
                             & \cdot
        \Abf(\overline{\vbf^*_T[1], \vbf^*_T[2], \ldots, \vbf^*_T[L - 1]} ; \overline{\vbf^*_T[1], \vbf^*_T[2], \ldots, \vbf^*_T[L - 1]}, \vbf^*_T[L])
    \end{split}
\end{equation}
\end{comment}

\begin{proof}
    Since the minimum length of prefix-sequence needed in order for the deviation of stepwise optimal response from the same-length global optimal response is $L$, then the advantage of the global optimal response is not manifested until step $L$.
    When $L > 2$, at the step $L - 1$ we have:
    \begin{equation}
        \small
        f(X_{1:L-1} = w_{\widehat{\vbf}_T[1]} w_{\widehat{\vbf}_T[1]} \ldots w_{\widehat{\vbf}_T[L - 1]} \mid X_{\leq 0})
        > f(X_{1:L-1} = w_{\vbf_T^*[1]} w_{\vbf_T^*[2]} \ldots w_{\vbf_T^*[L - 1]} \mid X_{\leq 0}),
    \end{equation}
    together with Assumption~\ref{aspt:well_trained_LLM}, we have:
    \begin{equation}
        \small
        \begin{split}
             & g(X_1 = w_{\widehat{\vbf}_T[1]} \mid X_{\leq 0}) ~ \Pi_{t = 1}^{L - 2} g(X_{t + 1} = w_{\widehat{\vbf}_T[t + 1]} \mid X_{1:t} = w_{\widehat{\vbf}_T[1]} w_{\widehat{\vbf}_T[2]} \ldots w_{\widehat{\vbf}_T[t]}, X_{\leq 0}) \\
             & > f(X_{1:L-1} = w_{\vbf_T^*[1]} w_{\vbf_T^*[2]} \ldots w_{\vbf_T^*[L - 1]} \mid X_{\leq 0}),
        \end{split}
    \end{equation}
    At the step $L$, we have:
    \begin{equation}
        \small
        f(X_{1:L} = w_{\widehat{\vbf}_T[1]} w_{\widehat{\vbf}_T[1]} \ldots w_{\widehat{\vbf}_T[L]} \mid X_{\leq 0})
        < f(X_{1:L} = w_{\vbf_T^*[1]} w_{\vbf_T^*[2]} \ldots w_{\vbf_T^*[L]} \mid X_{\leq 0}),
    \end{equation}
    together with Assumption~\ref{aspt:well_trained_LLM}, we have:
    \begin{equation}
        \small
        \begin{split}
             & g(X_1 = w_{\widehat{\vbf}_T[1]} \mid X_{\leq 0}) ~ \Pi_{t = 1}^{L - 1} g(X_{t + 1} = w_{\widehat{\vbf}_T[t + 1]} \mid X_{1:t} = w_{\widehat{\vbf}_T[1]} w_{\widehat{\vbf}_T[2]} \ldots w_{\widehat{\vbf}_T[t]}, X_{\leq 0}) \\
             & < f(X_{1:L} = w_{\vbf_T^*[1]} w_{\vbf_T^*[2]} \ldots w_{\vbf_T^*[L]} \mid X_{\leq 0}),
        \end{split}
    \end{equation}
    \begin{equation}
        \small
        \begin{split}
             & g(X_{t + 1} = w_{\widehat{\vbf}_T[t + 1]} \mid X_{1:t} = w_{\widehat{\vbf}_T[1]} w_{\widehat{\vbf}_T[2]} \ldots w_{\widehat{\vbf}_T[t]}, X_{\leq 0}) % \\
            % & < \frac{}{}
        \end{split}
    \end{equation}
    (clean-up in the process)
\end{proof}

\begin{comment}
Since the context length of the LLM is $N$, and the text generation takes a token-by-token format, one can write the conditional probability of generating the next token in terms of a transition probability of a 1-st order Markov process, where the transition is over the enhanced state space of all possible combinations of length-$N$ sequences:
\begin{equation}\label{equ:markov_transition}
    P(\overline{X_{t - N + 2} \ldots X_t} \, X_{t + 1} \mid X_{t - N + 1} \, \overline{X_{t - N + 2} \ldots X_t}) \coloneqq g(X_{t + 1} \mid X_{t - N + 1:t}).
\end{equation}
In the right-hand side of \eqnref{equ:markov_transition}, we use the overline notation $\overline{~\cdot~}$ to denote identical sub-sequences before and after state transition.
% The new state $\overline{X_{t - N + 2} \ldots X_t} \, X_{t + 1}$ is the length-$(N - 1)$ suffix of the previous state, i.e., $\overline{X_{t - N + 2} \ldots X_t}$, appended with the newly generated token $X_{t + 1}$.
Here, we are not imposing the assumption that the LLM with a context length of $N$ is a $(N + 1)$-gram model.
Instead, we use the transition matrix of the 1-st order Markov process over the enhanced state space (of length-$N$ sequences) to simplify the notation when characterizing the probability of generating a specific sequence.
Specifically, with a slight abuse of notation, let $\Abf([v_{t - N + 1 : t}]; [v_{t - N + 2 : t + 1}])$ denote entries in the transition matrix, which is indexed by two lists of vocabulary indices that form the from-sequence and to-sequence, respectively.
Let $\pi^{(t)}([v_{t - N + 1 : t}])$ denote the probability of reaching the state $w_{v_{t - N + 1}} w_{v_{t - N + 2}} \ldots w_t$ at the step $t$.

We can use $\pi^{(0)}$ to represent the initial condition specified by the prompt $X_{\leq 0}$ (after processed by the LLM).
Then, the probability of generating the next token $w_{v_{t + 1}}$ is the product of the distribution of states and the transition matrix:
\begin{equation}
    \pi^{(t + 1)}(v_{t - N + 2:t + 1})
    = \sum_{v_{t - N + 1 : t} \in \Vcal^N} \pi^{(t)}(v_{t - N + 1 : t}) \Abf(v_{t - N + 1 : t}; v_{t - N + 2 : t + 1}).
\end{equation}

If the current state is a length-$N$ sequence $X_{t - N + 1} \, \overline{X_{t - N + 2} \ldots X_t}$, then only when the next state starts with the length-$(N-1)$ suffix of the current state can the corresponding entries in the transition matrix to be nonzero.
We can denote with $\hat{v}_{t + 1}$ the index of the newly sampled token, given the previously sampled sequence $w_{\hat{v}_{t - N + 1}} w_{\hat{v}_{t - N + 2}} \ldots w_{\hat{v}_{t}}$:
\begin{equation}
    \hat{v}_{t + 1} = \argmax_{v_{t + 1}} \pi^{(t + 1)}(v_{t - N + 2:t} = \hat{v}_{t - N + 2:t}, v_{t + 1}).
\end{equation}

Since $L$ is the minimum length of prefix-sequence needed in order for the advantage of the global optimal length-$T$ response to manifest, we have:
\begin{equation}
    \begin{split}
        \forall t < L, f(X_{1:t} = w_{\hat{v}_1} w_{\hat{v}_2} \ldots w_{\hat{v}_t} \mid X_{\leq 0}) & > f(X_{1:t} = w_{\vbf^*[1]} w_{\vbf^*[2]} \ldots w_{\vbf^*[t]} \mid X_{\leq 0}), \\
        \text{and } f(X_{1:L} = w_{\hat{v}_1} w_{\hat{v}_2} \ldots w_{\hat{v}_L} \mid X_{\leq 0})    & < f(X_{1:L} = w_{\vbf^*[1]} w_{\vbf^*[2]} \ldots w_{\vbf^*[L]} \mid X_{\leq 0}).
    \end{split}
\end{equation}
In other words,
\begin{equation}
    \big( \pi^{(0)} \Abf \big)(\hat{v}_1) > \big( \pi^{(0)} \Abf \big)(\vbf^*_T[1]),
\end{equation}
\begin{equation}
    \big( \pi^{(1)} \Abf \big)(\hat{v}_1, \hat{v}_2) > \big( \pi^{(1)} \Abf \big)(\vbf^*_T[1], \vbf^*_T[2]),
\end{equation}
\begin{equation*}
    \ldots
\end{equation*}
\begin{equation}
    \big( \pi^{(L - 1)} \Abf \big)(\hat{v}_1, \hat{v}_2, \ldots, \hat{v}_{L - 1}) > \big( \pi^{(L - 1)} \Abf \big)(\vbf^*_T[1], \vbf^*_T[2], \ldots, \vbf^*_T[L - 1]),
\end{equation}
\begin{equation}
    \big( \pi^{(L)} \Abf \big)(\hat{v}_1, \hat{v}_2, \ldots, \hat{v}_L) < \big( \pi^{(L)} \Abf \big)(\vbf^*_T[1], \vbf^*_T[2], \ldots, \vbf^*_T[L]).
\end{equation}

We have
\begin{equation}
    \begin{split}
        \forall v \in \Vcal, & \Abf(\overline{\hat{v}_1, \hat{v}_2, \ldots, \hat{v}_{L - 1}} ; \overline{\hat{v}_1, \hat{v}_2, \ldots, \hat{v}_{L - 1}}, v)
        < \frac{\big( \pi^{(L - 1)} \Abf \big)(\vbf^*_T[1], \vbf^*_T[2], \ldots, \vbf^*_T[L - 1])}{\big( \pi^{(L - 1)} \Abf \big)(\hat{v}_1, \hat{v}_2, \ldots, \hat{v}_{L - 1})} \\
                             & \cdot
        \Abf(\overline{\vbf^*_T[1], \vbf^*_T[2], \ldots, \vbf^*_T[L - 1]} ; \overline{\vbf^*_T[1], \vbf^*_T[2], \ldots, \vbf^*_T[L - 1]}, \vbf^*_T[L])
    \end{split}
\end{equation}
\end{comment}

\cgy{Comments 1:  here, for a variable x1, we have three notations including x1 v1 wv1.}

\cgy{Suggestion 1: may we remove v, since w is already the value of variable x}

\cgy{Comments 2: for assumption 1.4, it is possible that $p(\hat{X}) < p(X^*) $ at length L, but then  $p(\hat{X}) = p(X^*) $ at length L+1. It is because, by definition, we only have $X^*$ is optimal for the whole sequence but may not be true at length L+1. }

\cgy{Question 2: is the assumption 1.4 necessary?}

\cgy{Comments 3: for theorem 1.5, why do we have a bound $1-\epsilon$? From the final equation, only $p(\hat{x}_{t+1})<p(x^{*}_{t+1})$ can be directly get.  Need more justifications. }

==> file/parking/relatedwork.tex <==

\section{Related Works}

This paper proposes a selective method to refine the text generation performance for large lauguage models (LLMs). There are multiple research directions related to it, such as LLM correction and refinement. In this section, we will discuss those related works, and highlight their differences from ours.  

\paragraph{Language Model Decoding Strategy} 

Despite significant progress in recent language model text generation, how to approach the optimal text decoding from a language model still remains an open question. The most commonly used decoding is maximization-based decoding, in which we always select the next token with highest conditional probability. \cite{holtzman2019curious} proposed a stochastic decoding method called Top-$p$ sampling (a.k.a. nucleus sampling), which utilized the shape of the probability distribution to determine the next-token set. Top-$k$ sampling \citep{radford2019language,holtzman2018learning,fan2018hierarchical} is a popular alternative method. The key difference between them is that: Top-$p$ sampling selects a subset of words that have a cumulative probability exceeding a certain threshold, while Top-$k$ sampling just selects a fixed number of top words. Another common approach is to shape a probability distribution through temperature \citep{caccia2018language,fan2018hierarchical,ficler2017controlling,ackley1985learning}.    
A line of works specify the language generation tasks as posterior inference problem and decode with sequential Monte Carlo sampling \citep{lew2023sequential,lew2023smcp3,zhi2024infinite}. Some papers aim to achieve fast inference via speculative decoding by computing several tokens in parallel \citep{leviathan2023fast,kim2024speculative,chen2023accelerating,xia2024unlocking,sun2024spectr,xia2023speculative}. Multiple works are based on beam search \citep{xie2024self,zhu2024deductive,wei2024confidence,yang2024language} for efficient inference.

\paragraph{Language Model Self-correction} Self-correction~\citep{pan2023automatically,shinn2023reflexion,yao2022react,madaan2023self,bai2022constitutional,ganguli2023capacity,chen2023teaching,kim2023language,tyen2023llms} refers to whether LLMs can refine their responses based on their previous outputs, leveraging either external or internal feedback. Numerous studies have demonstrated effective self-correction performance through the integration of external feedback generated by the learned critic models~\citep{paul2023refiner, akyurek2023rl4f, welleck2022generating,peng2023check,gao2023rarr} or interacting with human or tools~\citep{gou2023critic, chern2023factool, olausson2023self}. Training extra models or interacting with the real world may result in extra costs. Thus, recent studies are beginning to explore {intrinsic self-correction} \citep{li2024confidence,shinn2023reflexion,madaan2023self, chen2023iterative, manakul2023selfcheckgpt, huang2023large}, noted for its cost efficiency.


==> file/parking/table6.tex <==
% \begin{table*}[t]
%     \centering
%     \caption{Model Accuracy by Subject Category on MMLU Using Different Methods}
%     \label{tab:fullresult}
%     \begin{tabular}{lccc}
%     \toprule
%     \textbf{Category} & \textbf{Greedy (\%)} & \textbf{Beam Search (\%)} & \textbf{Ours (\%)} \\
%     \midrule
%     abstract\_algebra & 47.00 & 46.00 & 47.00 \\
%     anatomy & 67.40 & 74.07 & 72.59 \\
%     astronomy & 80.92 & 73.02 & 80.26 \\
%     business\_ethics & 66.00 & 68.00 & 64.00 \\
%     clinical\_knowledge & 76.22 & 76.60 & 78.11 \\
%     college\_biology & 83.33 & 80.55 & 79.86 \\
%     college\_chemistry & 56.00 & 53.00 & 57.00 \\
%     college\_computer\_science & 55.00 & 63.00 & 58.00 \\
%     college\_mathematics & 35.00 & 47.00 & 36.00 \\
%     college\_medicine & 69.36 & 65.89 & 68.78 \\
%     college\_physics & 64.70 & 69.61 & 61.76 \\
%     computer\_security & 73.00 & 78.00 & 77.00 \\
%     conceptual\_physics & 68.93 & 69.78 & 69.78 \\
%     econometrics & 56.14 & 58.77 & 57.89 \\
%     electrical\_engineering & 58.62 & 64.82 & 61.37 \\
%     elementary\_mathematics & 88.09 & 88.62 & 89.41 \\
%     formal\_logic & 50.00 & 50.79 & 51.58 \\
%     global\_facts & 43.00 & 45.00 & 50.00 \\
%     high\_school\_biology & 79.03 & 80.96 & 80.32 \\
%     high\_school\_chemistry & 62.07 & 67.98 & 63.05 \\
%     high\_school\_computer\_science & 81.00 & 79.00 & 79.00 \\
%     high\_school\_european\_history & 76.36 & 75.15 & 75.15 \\
%     high\_school\_geography & 78.79 & 80.81 & 78.79 \\
%     high\_school\_government\_and\_politics & 88.60 & 86.53 & 88.08 \\
%     high\_school\_macroeconomics & 69.74 & 74.62 & 68.97 \\
%     high\_school\_mathematics & 64.44 & 68.89 & 68.52 \\
%     high\_school\_microeconomics & 75.63 & 76.05 & 77.33 \\
%     high\_school\_physics & 54.97 & 54.97 & 57.62 \\
%     high\_school\_psychology & 85.32 & 88.07 & 86.24 \\
%     high\_school\_statistics & 62.96 & 60.19 & 62.96 \\
%     high\_school\_us\_history & 83.33 & 80.88 & 80.39 \\
%     high\_school\_world\_history & 78.90 & 80.59 & 76.79 \\
%     human\_aging & 63.68 & 66.82 & 62.78 \\
%     human\_sexuality & 52.67 & 60.31 & 53.44 \\
%     international\_law & 80.17 & 80.17 & 77.69 \\
%     jurisprudence & 72.22 & 74.07 & 76.85 \\
%     logical\_fallacies & 78.53 & 78.53 & 79.14 \\
%     machine\_learning & 56.25 & 61.61 & 53.57 \\
%     nutrition & 73.86 & 75.82 & 76.47 \\
%     us\_foreign\_policy & 84.00 & 80.00 & 81.00 \\
%     public\_relations & 64.55 & 66.36 & 65.45 \\
%     world\_religions & 83.04 & 79.53 & 82.46 \\
%     professional\_accounting & 51.42 & 53.98 & 51.06 \\
%     security\_studies & 62.45 & 66.12 & 63.27 \\
%     professional\_law & 49.86 & 51.54 & 53.50 \\
%     professional\_psychology & 68.63 & 68.95 & 68.46 \\
%     prehistory & 70.37 & 72.22 & 70.37 \\
%     professional\_medicine & 79.41 & 79.78 & 79.78 \\
%     sociology & 74.63 & 77.11 & 73.63 \\
%     philosophy & 73.06 & 68.49 & 71.40 \\
%     virology & 48.19 & 47.59 & 49.40 \\
%     marketing & 88.03 & 84.18 & 87.17 \\
%     medical\_genetics & 77.00 & 79.00 & 75.00 \\
%     miscellaneous & 86.97 & 87.73 & 87.61 \\
%     moral\_disputes & 67.34 & 66.76 & 64.16 \\
%     moral\_scenarios & 45.47 & 48.72 & 47.03 \\
%     \bottomrule
%     \end{tabular}
% \end{table*}

